Online Circle Packing

We consider the online problem of packing circles into a square container. A sequence of circles has to be packed one at a time, without knowledge of the following incoming circles and without moving previously packed circles. We present an algorithm that packs any online sequence of circles with a combined area not larger than 0.350389 0.350389 of the square's area, improving the previous best value of {\pi}/10 \approx 0.31416; even in an offline setting, there is an upper bound of {\pi}/(3 + 2 \sqrt{2}) \approx 0.5390. If only circles with radii of at least 0.026622 are considered, our algorithm achieves the higher value 0.375898. As a byproduct, we give an online algorithm for packing circles into a 1\times b rectangle with b \geq 1. This algorithm is worst case-optimal for b \geq 2.36.

==> 05-other.tex <==
In this section, we consider packing circles into a rectangle $R$ and prove our second main result:

\restatethm{\threctangleall*}{th:rectangle_all}

The idea is to use Double-Sided Structured Lane Packing (DSLP) to the lane~$R$. 


==> delta_2.tex <==
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[width=0.60\textwidth]{../../Bilder/placeholder.jpg}
%\end{figure}

%\begin{comment}
\begin{figure}[!htb]
	\centering
	\begin{minipage}[b]{0.495\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\begin{axis}[
		unbounded coords=jump,
		% A technical filter to cut out 
		% the x<0 and y<0 edge.
		filter point/.code={%
			\pgfmathparse
			{\pgfkeysvalueof{/data point/x}<0}%
			\ifpgfmathfloatcomparison
			\pgfmathparse
			{\pgfkeysvalueof{/data point/y}<0}%
			\ifpgfmathfloatcomparison
			\pgfkeyssetvalue{/data point/x}{nan}%
			\fi
			\fi
		},
		xtick={0.1,0.2,0.3,0.4,0.5},
		ytick={0.1,0.2,0.3,0.4,0.5},
		xmin = 0, xmax = 0.5,
		ymin = 0, ymax = 0.5,
		%x dir=reverse,
		%y dir=reverse
		point meta min=0.42, point meta max=1.3,xlabel={$r_1$},
		ylabel={$r_2$},zlabel={$\dlow_2(r_1,r_2)$}]
		\addplot3[surf,domain=0:0.5,domain y=0:0.5,samples=50] {pi/2*((x^2 + y^2)/(sqrt(2*1*(x+y)-1)*1)};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\begin{minipage}[b]{0.495\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\begin{axis}[
		unbounded coords=jump,
		% A technical filter to cut out 
		% the x<0 and y<0 edge.
		filter point/.code={%
			\pgfmathparse
			{\pgfkeysvalueof{/data point/x}<0}%
			\ifpgfmathfloatcomparison
			\pgfmathparse
			{\pgfkeysvalueof{/data point/y}<0}%
			\ifpgfmathfloatcomparison
			\pgfkeyssetvalue{/data point/x}{nan}%
			\fi
			\fi
		},
		xtick={0.1,0.2,0.3,0.4,0.5},
		ytick={0.1,0.2,0.3,0.4,0.5},
		xmin = 0, xmax = 0.5,
		ymin = 0, ymax = 0.5,
		%x dir=reverse,
		%y dir=reverse
		view={0}{90},
		point meta min=0.5, point meta max=1,xlabel={$r_1$},
		ylabel={$r_2$}]
		\addplot3[surf,domain=0:0.5,domain y=0:0.5,samples=50] {pi/2*((x^2 + y^2)/(sqrt(2*1*(x+y)-1)*1)};
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
\caption[Title]{Plots for the density bound function $\bmdelta_2(r_1,r_2)$. A global minimum is visually identifiable for some $r_1\in (0.2,0.4)$ and some $r_2\in (0.2,0.4)$.}\label{fig:delta_dim_plot}
\end{figure}
%\end{comment}

